User Support for the Combinator Logic Synthesizer Framework

Usability is crucial for the adoption of software development technologies. This is especially true in development stages, where build processes fail, because software is not yet complete or was incompletely modified. We present early work that aims to improve usability of the Combinatory Logic Synthesizer (CL)S framework, especially in these stages. (CL)S is a publicly available type-based development tool for the automatic composition of software components from a user-specified repository. It provides an implementation of a type inhabitation algorithm for Combinatory Logic with intersection types, which is fully integrated into the Scala programming language. Here, we specifically focus on building a web-based IDE to make potentially incomplete or erroneous input specifications for and decisions of the algorithm understandable for non-experts. A main aspect of this is providing graphical representations illustrating the step-wise search process of the algorithm. We also provide a detailed discussion of possible future work to further improve the understandability of these representations.

==> eptcsdata.tex <==
\providecommand{\firstpage}{16}
\providecommand{\publicationstatus}{P. Masci, R. Monahan, V. Prevosto (Eds.):  Formal\\
Integrated Development Environment 2018 (F-IDE 2018).\\
EPTCS 284, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.284.2}{10.4204/EPTCS.284.2}}
\pdfoutput=1

